Faster Guarantees of Evolutionary Algorithms for Maximization of Monotone Submodular Functions

In this paper, the monotone submodular maximization problem (SM) is studied. SM is to find a subset of size $\kappa$ from a universe of size $n$ that maximizes a monotone submodular objective function $f$. We show using a novel analysis that the Pareto optimization algorithm achieves a worst-case ratio of $(1-\epsilon)(1-1/e)$ in expectation for every cardinality constraint $\kappa < P$, where $P\leq n+1$ is an input, in $O(nP\ln(1/\epsilon))$ queries of $f$. In addition, a novel evolutionary algorithm called the biased Pareto optimization algorithm, is proposed that achieves a worst-case ratio of $(1-\epsilon)(1-1/e)$ in expectation for every cardinality constraint $\kappa < P$ in $O(n\ln(P)\ln(1/\epsilon))$ queries of $f$. Further, the biased Pareto optimization algorithm can be modified in order to achieve a worst-case ratio of $(1-\epsilon)(1-1/e)$ in expectation for cardinality constraint $\kappa$ in $O(n\ln(1/\epsilon))$ queries of $f$. An empirical evaluation corroborates our theoretical analysis of the algorithms, as the algorithms exceed the stochastic greedy solution value at roughly when one would expect based upon our analysis.

==> Sections/Theoretical/Pseudocode/add.tex <==

\begin{algorithm}
   \caption{\add$(\mathcal{S}, B', P, f)$}
   \label{algorithm:add}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definepool; $B'\subseteq U$; \defineP; \definef.
     \STATE {\bfseries Output:} \definepool.
     \IF{$|B'|< P$ and and $f(X)> f(\Sino{|B'|})$}
      \STATE $\mathcal{S} \gets \mathcal{S} \cup \{B'\}
              \setminus \Sino{|B'|}$
     \ENDIF
     \STATE \textbf{return} $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/bea_old.tex <==
\begin{algorithm}
   \caption{\bea$(f, P, T, p, \epsilon, \xi)$: \beal}
   \label{algorithm:bea}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definef; \defineP; \defineT; \definep;
     \defineepsilon; \definexi.
     \STATE {\bfseries Output:} \definepool.
     \STATE $M\gets\maxpointer$
     \STATE $\beta^i\gets 0$, $\ell_i\gets 0$, $H_i \gets e\ln(1/\epsilon)/\xi^i \: \forall i \in\{1,...,M\}$
     \STATE $\pool \gets $ \populate(\poolb, P)
     \FOR {$t\gets 1$ to $T$} \label{line:loopbea}
     \IF {$\flip(p)=$ heads}
     \STATE $i\gets\uniform(\{1,...,M\})$ \label{line:probp}
     \STATE $B\gets \Sino{\beta^i}$
     \STATE $B' \gets $ \mutate($B$) \label{line:mutate}
     \STATE $\mathcal{S} \gets \add(\mathcal{S}, B', P, f)$
     \STATE $\ell_i \gets \ell_i + 1$ \label{line:incell}
     \IF{$\ell_i = H_i$}
     \STATE $\ell_i\gets 0$ \label{line:ell}
     \IF{$\beta^i+1 < P$ and $f(\Sino{\beta^i+1})\geq f(\Sino{\beta^i})$} \label{line:condb}
     \STATE $\beta^i\gets \beta^i+1$ \label{line:probpend}
     \ENDIF
     \ENDIF
     \ELSE
     \STATE $B\gets\Sino{\uniform(\{0,...,P-1\})}$ \label{line:otherwise1}
     \STATE $B' \gets $ \mutate($B$)
     \STATE $\mathcal{S} \gets \add(\mathcal{S}, B', P, f)$ \label{line:otherwise2}
     \ENDIF
     \ENDFOR
     \STATE \textbf{return} $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/beasc.tex <==

\begin{algorithm}
   \caption{\beasc$(f, P, T, p, \epsilon, \xi)$: \beascl}
   \label{algorithm:beasc}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definef; \defineP; \defineT; \definep;
     \defineepsilon; \definexi.
     \STATE {\bfseries Output:} \definepool.
     \STATE $\mathcal S \gets \{ \emptyset \}$
     \STATE $\beta^i\gets 0$, $\ell_i\gets 0$, $H_i \gets e\ln(1/\epsilon)/\xi^i$ \alli
     \FOR {$t\gets 1$ to $T$}
     \STATE $B \gets $ \selectbeasc($\mathcal{S}, p, \beta^i$ \alli )
     \STATE $B' \gets $ \mutate($B$)
     \STATE $\mathcal{S} \gets \add(\mathcal{S}, B', P, f)$
     \IF{$\exists i$ s.t. $|B|=\beta^i$}
     \STATE $\ell_i \gets \ell_i + 1$ \label{line:incellsc}
     \IF{$\ell_i = H_i$}
     \STATE $\ell_i\gets 0$ \label{line:ellsc}
     \IF{$\exists X\in\mathcal{S}$ such that $|X|=\beta^i+1$ and $f(X)\geq f(B)$}
     \STATE $\beta^i\gets \beta^i+1$
     \ENDIF
     \ENDIF
     \ENDIF
     \ENDFOR
     \STATE \textbf{return} $\mathcal{S}$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/populate.tex <==

\begin{algorithm}
   \caption{\populate($\mathcal{S}, P$): Populate Algorithm}
   \label{algorithm:populate}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definepool, \defineP.
     \STATE {\bfseries Output:} \definepool.
     \STATE \textbf{return} \poolb
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/selectbea.tex <==

\begin{algorithm}
   \caption{\selectbea($P,p,\beta^i$ \allishort): Selection Algorithm for \bea}
   \label{algorithm:selectbea}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \defineP;
     \definep; $\beta^i\in\{0,...,n\}$ \allishort.
     \STATE {\bfseries Output:} $j\in\cardsno$
     \STATE With probability $p$, choose $j$ uniformly randomly among
            $\beta^i$ \allishort;
            otherwise, choose $j$ uniformly randomly among
            $\cardsno$.
     \STATE \textbf{return} $j$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/selectbea_old.tex <==

\begin{algorithm}
   \caption{\selectbea($\mathcal{S},p,\beta^i$ \alli): Selection Algorithm for \bea}
   \label{algorithm:selectbea}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definepool s.t. \alli $\exists X\in\mathcal{S}$ where $|X|=\beta^i$;
     \definep; $\beta^i\in\{0,...,n\}$ \alli.
     \STATE {\bfseries Output:} \defineB
     \STATE With probability $p$, choose $\beta$ uniformly randomly among
            $\beta^i$ \alli
            and let $B$ be the set in $\mathcal S$ such that $|B|=\beta$;
            otherwise, with probability $(1-p)$, choose uniformly randomly among the
            elements of $\mathcal S$.
     \STATE \textbf{return} $B$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/selectbeasc.tex <==

\begin{algorithm}
   \caption{\selectbeasc($\mathcal{S},p,\beta^i$ \alli): Selection Algorithm for \beasc}
   \label{algorithm:selectbeasc}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \definepool s.t. \alli $\exists X\in\mathcal{S}$ where $|X|=\beta^i$;
     \definep; $\beta^i\in\{0,...,n\}$ \alli.
     \STATE {\bfseries Output:} \defineB
     \STATE With probability $p$, choose $\beta$ uniformly randomly among
            $\beta^i$ \alli
            and let $B$ be the set in $\mathcal S$ such that $|B|=\beta$;
            otherwise, with probability $(1-p)$, choose uniformly randomly among the
            elements of $\mathcal S$.
     \STATE \textbf{return} $B$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Pseudocode/selectea.tex <==

\begin{algorithm}
   \caption{\selectea($P$): Selection Algorithm for \ea}
   \label{algorithm:selectea}
   \begin{algorithmic}[1]
     \STATE {\bfseries Input:} \defineP.
     \STATE {\bfseries Output:} $j\in\cardsno$.
     \STATE \textbf{return} a uniformly randomly chosen $j\in\cardsno$
\end{algorithmic}
\end{algorithm}


==> Sections/Theoretical/Theorems/bea_old.tex <==
\begin{theorem}
  \label{theorem:bea}
  Suppose we run \bea with input monotone submodular \definef
  \defineP, \definep, \defineepsilon, and \definexi.
  For any $\kappa < P$, if \poolb is the pool of \bea at the end of iteration
  $T\geq\max\{\alpha n\maxpointer, \beta\ln(n)\maxpointer\}$, where $\alpha=2e\ln(1/\epsilon)/p$
  and $\beta=8/p$ ,
  of the for loop of \bea then
  $$\ex{\max_{X\in\mathcal{S}, |X|\leq \kappa}f(X)}
   \geq (1-1/n)(1-1/e-\epsilon)\max_{|X|\leq \kappa}f(X).$$
\end{theorem}

\begin{proof}
  Proofs of lemmas used can be found in Appendix \ref{appendix:bealemmas}.
  Lines numbers referenced are those in Algorithm \ref{algorithm:bea}.
  Throughout the proof of Theorem \ref{theorem:bea}, the probability space
  of all possible runs of \bea with the stated inputs is considered. An iteration of the
  for loop in \bea is simply referred to as an iteration.

  Consider any $\kappa < P$. Define $A^*=\argmax_{|X|\leq \kappa}f(X)$. Without loss of
  generality we may assume that $|A^*|=\kappa$.
  There exists $q\in\{1,...,\maxpointer\}$ such that
  \begin{align}
    \xi^qP < |A^*| \leq \xi^{q-1}P. \label{eqn:boundopt}
  \end{align}
  %For notational simplicity, we define $\beta = \beta^q$ and $\ell=\ell_q$.
  %where the definition of $\beta^q$ can be found in the pseudocode for
  %\beasc (Algorithm \ref{algorithm:beasc}).

  %Recall the definitions of the variable $\omega$ from the
  %analysis of \ea (Theorem \ref{theorem:ea} in Section \ref{section:eaanalysis}).
  %For $\omega$ to be incremented during an iteration, $\Sino{\beta}$ must be selected
  %to be mutated.
  %This occurs with probability $1/P$.
  %In order to have the approximation guarantee presented in Theorem \ref{theorem:ea},
  %$\omega$ must increase to $\kappa$.
  %If we instead consider an alternative version of \ea where the selection is biased
  %towards choosing $X$ with constant probability $p$, then the expected time of \ea until $\omega$
  %towards picking $\Sino{\beta}$ with greater probability, then $\omega$ could increase to
  %$\kappa$ faster.
  %then the expected time of \ea until $\omega$
  %reaches \budget can be sped up by a factor of $p\kappa$.
  %reaches \budget can be sped up.
  %The difficulty is that the value of $\beta$ is unknown, since it depends on
  %The difficulty is that we cannot identify $X$ in \poolb unless we know $A^*$.
  %The difficulty is that in order to say the value of $\beta$ during \ea
  %it is required that we know whether
  %\mutate flipping the membership of some $a^*\in A^*$.
  %The idea behind \bea is that we can \textit{approximately} track $\beta$, and therefore
  %bias the selection.
  %and therefore the selection process biased,
  %with a small loss to the approximation guarantee and feasibility.
  %In particular, the approximate $\beta$ is $\beta^q$, which is selected
  %to be mutated with probability \beaprobsh where $M=\maxpointer$.
  %The reason we are biased towards $\beta^1,...,\beta^M$ instead of just $\beta^q$
  %is because $\beta^q$ depends on $\kappa$ (see Equation \ref{eqn:boundopt}) but we want
  %approximation guarantees for any cardinality constraint.
  %With this in mind, we re-define the variables $\omega$ and $\beta$ inductively as follows:
  %The idea behind \bea is that if
  %the set $X\in\pool$ such that $|X|=\beta$ is chosen \Hequal many times, then
  %we can say with high probability that on at least one of those times \mutate resulted
  %in the flipped membership of a single $a^*\in A^*$ and no other changes. Therefore
  %$\beta$ can be approximately tracked and therefore the selection process biased.
  %This results in a small loss to the approximation guarantee.
  %With this in mind, we re-define the variables $\omega$ and $\beta$ inductively as follows:
  TODO: Discussion for intuition compared to \ea.
  For notational simplicity we define $\omega$ to be $\omega^q$, $H=H_q$, and $\ell=\ell_q$.
  %\begin{itemize}[noitemsep]
  %  \item[(i)] Before the first iteration, $\omega=0$.
  %  \item[(ii)] $\omega$ is incremented at the end of an iteration if
  %  $q$ has been returned on Line \ref{line:random}
    %$B=\Sino{\beta}$ has been selected to be mutated on
    %the element $B\in\mathcal{S}$ of cardinality $\beta^q$
    %has been returned by \selectbea
  %  \Hq iterations since the last time $\omega$
  %  was incremented. E.g. the variable $\ell_q$ of Algorithm \ref{algorithm:bea}
  %  is set to 0 (Line \ref{line:ell} if $i=q$).
  %  \item[(iii)] $\beta$ is incremented if $\omega$ is incremented,
  %  $\beta+1<P$, and $f(\Sino{\beta+1})\geq f(\Sino{\beta})$. E.g.
  %  the conditions of Line \ref{line:condb} of Algorithm \ref{algorithm:bea} are met
  %  for $i=q$.
  %\end{itemize}
  %Notice that $\beta=\beta^q$.
  %The second condition on incrementing $\beta$ is to ensure that the solution quality
  %of the element in $\pool$ of cardinality $\beta$ is always improving.
  %Notice that $\beta$ is the same as $\beta^q$, but is re-defined for notational simplicity.
  %The definition of $\beta$ is the same as that found in the description of \bea.
  The $\omega$ defined here serves a similar purpose to that defined in the
  proof of Theorem \ref{theorem:ea}; To track a solution within
  $\mathcal{S}$ that has a high $f$ value relative to its cardinality, as described in
  the following lemma.
  \begin{lemma}
    \label{lemma:expectationbea}
    %Throughout the duration of \bea it is the case that $\beta\leq\omega$ and
    At the end of every iteration of \bea
    $$\ex{\maxf{\omega}} \geq \left(1-\left(1-\frac{1-\epsilon}{|A^*|}\right)^{\omega'}\right)f(A^*)$$
    where $\omega'=\min\{\omega,P-1\}$.
    \end{lemma}
  %Notice that Lemma \ref{lemma:expectationbea} is different compared to Lemma
  %\ref{lemma:expectation} because of the $\epsilon$. This is because
  %when $\omega$ is incremented we can only say with high probability
  %that on at least one of those times \mutate resulted
  %in the flipped membership of a single $a^*\in A^*$ and no other changes as
  %mentioned above.

  \noindent Because \bea and \ea share the same \add procedure, the property of
  \ea detailed in Lemma \ref{lemma:replace} of Theorem \ref{theorem:ea}
  also hold for \bea. That is, once a solution appears in the pool of \bea with the
  properties described in Lemma \ref{lemma:expectationbea}, that solution is never replaced with
  a solution that does not have that property.

  Define the event $F$ to be that at the
  completion of a run of \bea $\ell$ has been incremented (Line \ref{line:incell}
  of Algorithm \ref{algorithm:bea})
  $H\kappa$ times.
  If $\ell$ has been incremented $H\kappa$ times, then one may see that $\omega$ has been incremented
  $\kappa$ times. Once $\omega$ reaches $\kappa$, it clearly follows
  from Lemmas \ref{lemma:expectationbea} and \ref{lemma:replace} that
  \begin{align}
    \ex{f(A)|F} \geq \left(1-\frac{1}{e}-\epsilon\right)f(A^*) \label{eqn:hfd666}
  \end{align}
  where $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq\kappa}f(X)$.

  We now analyze the probability that $\ell$ has been incremented $H\kappa$ times.
  To this end, we have the following lemma.
  \begin{lemma}
    \label{lemma:bernoullibea}
    Consider a run of \bea as a series of Bernoulli trials $Y_1,...,Y_T$,
    where each iteration is a
    trial and a success is defined to be when $\ell$ is incremented.
    Then $Y_1,...,Y_T$ are independent, identically distributed Bernoulli trials where the
    probability of success is \beaprob.
  \end{lemma}

  Finally, an analogous argument to that of Theorem \ref{theorem:ea} can be used to
  complete the proof of Theorem \ref{theorem:bea}.
  In particular, we bound the probability of event $F$ not occurring after
  $T\geq\max\{\alpha n\maxpointer, \beta\ln(n)\maxpointer\}$, where $\alpha=2e\ln(1/\epsilon)/p$
  and $\beta=8/p$,
  iterations of \bea by $1/n$ using the Chernoff bound, and then apply the law of total
  probability.
  The details of the argument can be found in Section \ref{appendix:bealemmas}.
\end{proof}











%













%


==> Sections/Theoretical/Theorems/beasc.tex <==
\begin{proof}
  The probability space of all possible runs of \beasc with the stated inputs is considered.
  There exists some fixed $q\in\{1,...,\maxpointer\}$ such that
  \begin{align}
    \xi^qn < |A^*| \leq \xi^{q-1}n. \label{eqn:boundopt}
  \end{align}
  Define $\beta = \beta^q$, where the definition of $\beta^q$ can be found in the pseudocode for
  \beasc (Algorithm \ref{algorithm:beasc}).
  $\omega$ is defined analogously as in the proof of
  Theorem \ref{theorem:bea}:
  \begin{itemize}[noitemsep]
    \item[(i)] Before the first iteration, $\omega=0$.
    \item[(ii)] $\omega$ is incremented at the end of an iteration if
    $\ell_q$ is set to 0 (Line \ref{line:ellsc} of Algorithm \ref{algorithm:beasc}).
  \end{itemize}
  Refer to the proof of Theorem \ref{theorem:bea} for the definitions of
  $\omega_i$, $\beta_i$, and $X_i$.

  The result of Lemma \ref{lemma:expectationbpo} can be shown to hold for the current
  context using the exact same argument with the exception of Equation \ref{eqn:prob}.
  Instead, in order to have the result of Equation \ref{eqn:prob}, one must notice that
  \begin{align*}
    P(\neg F|E) \overset{a}{\leq} \left(1-\frac{|A^*|}{en}\right)^{H_q}
    \overset{b}{\leq} \epsilon
  \end{align*}
  where (a) is using Lemma \ref{lemma:beaprobevent}; and
  (b) is using that $H_q=\ln(1/\epsilon)/\xi^q$ and $n\xi^q<|A^*|$.

  \begin{lemma}
      \label{lemma:successbeasc}
      At the beginning of an iteration of \beasc, the probability
      that $\ell_q$ will be incremented
      during that iteration is
      $p/\left(\maxpointer\right)$.
    \end{lemma}
    \begin{proof}
      This is clear from looking at \selectbeasc.
    \end{proof}

  Let event $F$ be that at the completion of a run of \beasc, $\ell_q$ has been
  incremented $H_q\ln(1/\delta)/(1-\epsilon)|A^*|$
  many times (Line \ref{line:incellsc} of Algorithm \ref{algorithm:beasc}).
  If $\ell_q$ has been incremented $H_q\ln(1/\delta)/(1-\epsilon)|A^*|$
  many times, then one can see that $\omega\geq\min\{n,\ln(1/\delta)/(1-\epsilon)|A^*|\}$.
  %\todo{} Handle $\omega=n$ case.
  Let $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq\ln(1/\delta)/(1-\epsilon)|A^*|}f(X)$. Then
  \begin{align}
    \ex{f(A)|F} &\overset{a}{\geq}
    \left(1-\left(1-\frac{1-\epsilon}{|A^*|}\right)^{\ln(1/\delta)/(1-\epsilon)|A^*|}\right)f(A^*) \nonumber \\
    &\geq (1-\delta)\tau. \label{eqn:ksj3422}
  \end{align}
  where (a) is by an analogous argument to that used in Theorem \ref{theorem:ea} but
  instead using Lemma \ref{lemma:expectationbpo}.

  We now apply Chernoff's Bound in order to bound the probability of event
  $F$ not occurring.
  Again, a run of \beasc is considered as a
  series of independent Bernoulli trials: Each
  iteration is a trial and it is a success if $\ell_q$ is incremented. Let the random variable
  associated with iteration $i$ be $Y_i$.
  Then Chernoff's bound (Lemma \ref{lemma:chernoff}) as well as the fact that
  \beascT, can be used to show that
  \begin{align}
    P\left(\sum_{i=1}^TY_i < H_q\frac{\ln(1/\delta)|A^*|}{1-\epsilon}\right) \leq \delta. \label{eqn:dspe30}
  \end{align}
  where details are given in Lemma \ref{lemma:chernoffbeasc}.
  Finally, the Law of Total Probability along with Equations \ref{eqn:ksj3422} and \ref{eqn:dspe30}.
  gives the result stated in Theorem \ref{theorem:beasc}.
\end{proof}





















%


==> Sections/Theoretical/Theorems/ea_old.tex <==
\begin{theorem}
  \label{theorem:ea}
  Suppose we run \ea with input monotone submodular \definef
  and \defineP.
  For any $\kappa < P$, if \poolb is the pool of \ea at the end of iteration
  $\eaT$ of the for loop of \ea then
  $$\ex{\max_{X\in\mathcal{S}, |X|\leq \kappa}f(X)}
   \geq (1-1/n)(1-1/e)\max_{|X|\leq \kappa}f(X).$$
\end{theorem}

\begin{proof}
Proofs of lemmas used can be found in Appendix \ref{appendix:ealemmas}.
Lines numbers referenced are those in Algorithm \ref{algorithm:ea}.
An iteration of the
for loop in \ea is simply referred to as an iteration.
Throughout the proof of Theorem \ref{theorem:ea}, the probability space
of all possible runs of \ea with the stated inputs is considered.

Consider any $\kappa < P$. Define $A^*=\argmax_{|X|\leq \kappa}f(X)$. Without loss of
generality we may assume that $|A^*|=\kappa$.
In the proof of Theorem \ref{theorem:ea}, two variables, $\omega$ and $\beta$,
are tracked. They are defined inductively as follows:
\begin{itemize}[noitemsep]
  \item[(i)] Before the first iteration of \ea, $\omega=\beta=0$.
  \item[(ii)] $\omega$ is incremented at Line \ref{line:beforeremove}
  if the following two conditions are met during the iteration:
  $B=\Sino{\beta}$ is selected on Line \ref{line:selectea}; and \mutate results in
  the membership of a single element $a^*\in A^*$ being flipped
  (i.e. it is either the case that \mutate returns $B'=B\cup\{a^*\}$ for $a^*\in A^*\setminus B$
  or $B'=B\setminus\{a^*\}$ for $a^*\in A^*\cap B$).
  \item[(iii)] $\beta$ is incremented at Line \ref{line:beforeremove}
  if the following
  three conditions are met during that iteration: $\beta<P-1$;
  $\omega$ was also
  incremented during the iteration; and the flipped membership element $a^*\in A^*$
  described in (ii) was added
  (i.e. \mutate returns $B'=B\cup\{a^*\}$ for $a^*\in A^*\setminus B$).
  \item[(iv)] $\beta$ is decreased to $\max\{i: i\leq\beta, \Sino{i} \text{ exists}\}$
  (notice that it is always the case that at least $0\in\{i: i\leq\beta, \Sino{i} \text{ exists}\}$)
  at Line \ref{line:afterremove}
  if on Line \ref{line:remove} a set $Y$ is removed from \poolb such that $|Y|=\beta$.
  %If $\Sino{\beta}$ does not exist at the end of an iteration, then
  %$\beta$ is set to be $\max\{i: i\leq\beta, \Sino{i} \text{ exists}\}$.
\end{itemize}
%Intuitively, throughout \ea there always exists exactly one element in $\mathcal{S}$
%of cardinality $\beta$, and that element has an approximation guarantee relative to the
%optimum. This is formally stated in the following lemma.
%The key point of the argument of Theorem \ref{theorem:ea} is that as long as
%$\omega < P$ in \ea,
%there exists $X\in\pool$ such that $|X|=\beta$
%and $f(A^*)-\ex{f(X)} \leq \left(1-1/\kappa\right)^{\omega}f(A^*)$.
%and has an approximation guarantee relative to the optimum.
%Further, $\omega$ increases monotonically to \budget in expected \eatime time,
%combined with the Chernoff bound (Lemma \ref{lemma:chernoff} of Section
%\ref{appendix:theoretical} in the appendix) which gives the
%result of Theorem \ref{theorem:ea}.
%The key properties of $\omega$ and $\beta$ for the proof of Theorem \ref{theorem:ea}
%are presented in the following lemma.
Intuitively, $\omega$ and $\beta$ are used to track a solution within
$\mathcal{S}$ that has a high $f$ value relative to its cardinality.
In particular, the following lemma describes the
key property of $\omega$ and $\beta$.
\begin{lemma}
  \label{lemma:expectation}
  At the end of every iteration of \ea
  %it is the case that $\beta\leq\omega$ and
  $\Sino{\beta}$ exists, $\beta\leq\omega$, and
  $$\ex{f(\Sino{\beta})} \geq \left(1-\left(1-\frac{1}{|A^*|}\right)^{\min\{\omega,P-1\}}\right)f(A^*).$$
\end{lemma}
%\begin{proof} Included in Appendix \ref{appendix:ealemmas}.\end{proof}
\noindent A further key point is that once a solution appears in the pool of \ea with the
properties described in Lemma \ref{lemma:expectation}, that solution is never replaced with
a solution that does not have that property. This follows from the following lemma.
\begin{lemma}
  \label{lemma:replace}
  If at the beginning of iteration $i$ there exists
  $X\in\mathcal{S}$ such that $|X|\leq a$ and $f(X) \geq b$.
  Then at the end of iteration $j\geq i$ there exists
  $Y\in\mathcal{S}$ such that $|Y|\leq a$ and $f(Y) \geq b$.
\end{lemma}

  \noindent Let event $F$ be that at the completion of a run of \ea, $\omega\geq \kappa$.
  Then it clearly follows from Lemmas \ref{lemma:expectation} and \ref{lemma:replace}
  that
  \begin{align}
    \ex{\max_{X\in\mathcal{S}, |X|\leq \kappa}f(X)|F}
    \geq \left(1-\frac{1}{e}\right)f(A^*) \label{eqn:hfd66672}
  \end{align}
  where $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq\kappa}f(X)$. Then the remainder of the
  proof of Theorem \ref{theorem:ea} is to deal with the probability that $\omega$
  reaches $\kappa$.
  To this end, the following
  lemma states that the entire run of \ea is a Bernoulli process.
  \begin{lemma}
    \label{lemma:bernoulli}
    Consider a run of \ea as a series of Bernoulli trials $Y_1,...,Y_T$,
    where each iteration is a
    trial and a success is defined to be when $\omega$ is incremented.
    Then $Y_1,...,Y_T$ are independent, identically distributed Bernoulli trials where the
    probability of success is
    \begin{align*}
      \frac{1}{P}\sum_{x\in A^*}\left(1-\frac{1}{n}\right)^{n-1}\frac{1}{n} \geq \frac{|A^*|}{enP}.
    \end{align*}
  \end{lemma}
  \noindent Then Lemma \ref{lemma:bernoulli} and the Chernoff bound can be used to prove that the
  probability of $\omega$ not reaching $\kappa$ after $T\geq\eaT$
  iterations of \ea is small. This is stated in the following lemma.
  \begin{lemma}
    \label{lemma:probability}
    \begin{align*}
      P\left(\sum_{i=1}^TY_i < \kappa\right) \leq \frac{1}{n}.
    \end{align*}
  \end{lemma}
  \noindent Finally, the Law of Total Probability along with Equation \ref{eqn:hfd66672} and
  Lemma \ref{lemma:probability}
  prove Theorem \ref{theorem:ea}.
\end{proof}











%


==> Sections/Theoretical/Theorems/easc.tex <==
\begin{theorem}
  \label{theorem:easc}
  Suppose we run \ea with input monotone submodular \definef
  and $P=n+1$.
  Then for any $\tau \leq f(U)$ and \definedelta
  if \poolb is the pool of \ea at the end of iteration
  \eascT of the for loop of \ea then
  $$\ex{\max_{X\in\mathcal{S}, |X|\leq \ln(1/\delta)|A^*|}f(X)}
   \geq (1-1/n)(1-\delta)\tau.$$
\end{theorem}

\begin{proof}
  Consider any $\tau\leq f(U)$. Define $A^*=\argmin_{f(X)\geq\tau}|X|$.
  $\omega$ and $\beta$ are defined in the same way as in the proof of Theorem
  \ref{theorem:ea}.
  Then Lemmas \ref{lemma:expectation}, \ref{lemma:replace}, and \ref{lemma:bernoulli}
  in the proof of Theorem \ref{theorem:ea} also hold in this context.
  The proof of Theorem \ref{theorem:easc} proceeds in the same manner as the proof of
  Theorem \ref{theorem:ea}, except we analyze the event that $\omega$ reaches
  $\ln(1/\delta)|A^*|$ instead of $|A^*|.$

  Let event $F$ be that at the completion of a run of \ea, $\omega\geq\ln(1/\delta)|A^*|$.
  Then it clearly follows from Lemmas \ref{lemma:expectation} and \ref{lemma:replace}
  that
  \begin{align}
    \ex{\max_{X\in\mathcal{S}, |X|\leq \ln(1/\delta)|A^*|}f(X)}
    \geq (1-1/n)(1-\delta)\tau. \label{eqn:ksj2}
  \end{align}
  Then the probability of event $F$ not occurring after
  \eascT
  iterations of \bea can be bounded
  by $1/n$ using the Chernoff bound, and then the law of total
  probability applied.
  The details of the argument can be found in Section \ref{appendix:bealemmas}.

%  $\omega\geq \min\{n,\ln(1/\delta)|A^*|\}$.
%  Define $$A=\text{argmax}_{X\in\mathcal{S}, |X|\leq\ln(1/\delta)|A^*|}f(X).$$
%  Then by a similar argument to that used to prove Equation \ref{eqn:hfd66672} of
%  Theorem \ref{theorem:ea}, it can be shown that
%  \begin{align}
%    \ex{f(A)|F} &\geq \ex{f(X_t)|F} \nonumber \\
%    &\geq (1-\delta)\tau. \label{eqn:ksj2}
%  \end{align}
%  In addition, as in the proof of Theorem \ref{theorem:ea}, a run of \ea is considered as a
%  series of independent Bernoulli trials: Each
%  iteration is a trial and it is a success if $\omega$ is incremented. Let the random variable
%  associated with iteration $i$ be $Y_i$, hence $Y_i=1$ if $\omega$ is incremented at iteration $i$
%  and $Y_i=0$ otherwise.
%  Then Chernoff's bound (Lemma \ref{lemma:chernoff}) as well as the fact that
%  $T\geq\max\{2en^2\ln(1/\delta), 8en^2\ln(1/\delta)\}$, can be used to show that
%  \begin{align}
%    P\left(\sum_{i=1}^TY_i < \min\{n,\ln\left(\frac{1}{\delta}\right)|A^*|\}\right)
%    \leq \delta. \label{eqn:3dgy}
%  \end{align}
%  where the details may be found in Lemma \ref{lemma:chernoffeasc}.
%  Finally, Equations \ref{eqn:ksj2} and \ref{eqn:3dgy} along with the Law of Total
%  Probability prove the result of Theorem \ref{theorem:easc}.
\end{proof}


==> Sections/Theoretical/bea_old.tex <==
\beal (\bea) is a novel evolutionary algorithm with nearly the same approximation
results as \ea for SM, but in this section it is proven that
\bea finds a \bearatio approximate solution in expectation in \beatimenop time.
Despite \bea being faster than \ea by a factor of \budget, \bea is only different
from \ea in that its selection procedure is biased instead of choosing uniformly
randomly.
%The algorithm \bea is described in Section \ref{section:beaoverview} and pseudocode
%for \bea is provided in Algorithm \ref{algorithm:bea}.

\subsubsection{Description of \bea}
\label{section:beaoverview}
\input{Sections/Theoretical/Pseudocode/bea}
\input{Sections/Theoretical/Pseudocode/selectbea}
The novel algorithm \bea is presented in Algorithm \ref{algorithm:bea}.
\bea follows a similar iterative procedure to \ea.
%and therefore only the differences between \bea and \ea will be described here.
%\bea (Algorithm \ref{algorithm:bea}) follows a similar iterative procedure to \ea,
%and therefore only the differences between \bea and \ea will be described here.
%In addition to the parameters of \ea, \bea requires parameters \definep and
%\defineH.
Instead of the procedure \selectea where a solution is
chosen uniformly randomly from $\pool$, \bea has the procedure \selectbea
(Algorithm \ref{algorithm:selectbea}) that is
biased towards a specific solution in $\pool$.
In particular, \bea keeps track of a variable $\beta$.
\selectbea returns the element in $\pool$ of cardinality $\beta$ with probability $p$,
and otherwise returns an element uniformly randomly from $\pool$.
Initially, $\beta=0$.
$\beta$ is incremented to $\beta+1$ if (i) there exists as $X\in\pool$ such that
$|X|=\beta+1$ with sufficiently high $f(X)$, and (ii)
on $H$ iterations since the last increment of $\beta$ \selectbea has chosen
the element in $\pool$ of cardinality $\beta$ (the variable $\ell$ in Algorithm
\ref{algorithm:selectbea} is used to determine when $\beta$ should be incremented).
Notice that if $p=0$, \bea is equivalent to \ea.

\subsubsection{Analysis of \bea for SM}
\label{section:beaanalysis}
The approximation results of \bea for SM are now presented.
\bea uses some definitions and lemmas from the proof of Theorem \ref{theorem:ea}
in Section \ref{section:eaanalysis}, and the reader should refer to these sections
if needed. Lemmas referenced in the proof of Theorem \ref{theorem:bea} can be found in
Section \ref{appendix:theoretical} of
the appendix.

\input{Sections/Theoretical/Theorems/bea}


















%


==> Sections/Theoretical/beasc.tex <==
\beascl (\beasc) is a version of \bea for SC that does not require knowledge of $|A^*|$.
It is proven in Section \ref{section:beascanalysis} that \beasc finds approximate solutions that are
near feasible in expectation for SC in \beasctime time.
To the best of our knowledge, there does not yet exist an \sg analogue proposed for
SC, and thus \beasc is the first \beasctime time algorithm analyzed for SC.
\beasc is like \bea, but is biased towards \maxpointersimple many solutions in
its pool, each corresponding to an estimate of $|A^*|$.
The algorithm \beasc is described in Section \ref{section:beascoverview} and pseudocode
for \beasc is provided in Section \ref{appendix:beasc} in the appendix.

\subsubsection{Overview of \beasc}
\label{section:beascoverview}
\beasc (Algorithm \ref{algorithm:beasc} in Section \ref{appendix:beasc} in the appendix)
is similar to \bea, and therefore only the differences between \beasc and \bea
are described here.
In addition to the parameters of \bea, \beasc requires the parameter \definexi.
\beasc keeps track of variables $\beta^i$ \alli.
\selectbeasc returns an element of $\pool$ of cardinality $\beta^i$, where $i$ is chosen
uniformly randomly (there always exists one), with probability $p$,
and otherwise chooses uniformly randomly from $\pool$.
Initially, $\beta^i=0$ \alli.
$\beta^i$ is incremented when the following conditions have been met on \Hi many times:
\selectbeasc results in the selection of the element in $\pool$ is cardinality
$\beta^i$, and \mutate resulted in the flipped membership of a
single element.
The details of \beasc, as well as the subroutine \selectbeasc
can be found in Algorithm \ref{algorithm:beasc} of Section \ref{appendix:beasc} in the appendix.
It should be noted that \beasc is not equivalent to running a separate \bea with $\beta=\beta^i$ for
each $i$, because there is one pool $\pool$ that is being shared.

\subsubsection{Analysis of \beasc for SC}
\label{section:beascanalysis}
The approximation results of \beasc for SC are now presented.
In contrast to Theorem \ref{theorem:bea}, it is the feasibility that is in expectation.
\begin{theorem}
  \label{theorem:beasc}
  Suppose we have an instance of SC with optimal solution $A^*$ such that
  $|A^*|\geq 2$.
  Let $P=n$, $\delta\in(0,1]$, \defineepsilon, \definexi, and \beascT
  Then if \ea is run with
  these inputs and $\mathcal{S}$ is its pool at completion,
  $\ex{f(A)} \geq (1-1/n)(1-\delta)\tau$
  where
  $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq \ln(1/\delta)/(1-\epsilon)|A^*|}f(X).$
\end{theorem}
Recall that in \bea in Section \ref{section:bea} that $\beta$ is advanced if $\ell$ has been
incremented $n/\kappa\ln(1/\epsilon)$ many times.
A difficulty with applying \bea to SC is that the cardinality of the optimal solution
(\budget in SM) is unknown.
This difficulty is ameliorated in \beasc by making $\maxpointer$ guesses for $|A^*|$,
each with a corresponding $\beta_i$. The $\beta_i$ corresponding to the closest
lower bound of $|A^*|$ is chosen with probability $p/\maxpointer$, resulting in a
$\maxpointer$ slow down compared to \bea.

\input{Sections/Theoretical/Theorems/beasc}
























%


==> Sections/Theoretical/cover.tex <==
In this section, we briefly present approximation results on the closely related
Submodular Cover (SC) Problem.
Additional details and proofs can be found in Section \ref{appendix:cover} in the appendix.
SC is defined as follows.
\begin{problem}[Submodular Cover Problem (SC)]
  Let \definef be a monotone submodular function
  defined on subsets of the ground set $U$ of size $n$.
  Given a threshold
  $\tau\in [0,f(U)]$, SC is to find $\text{argmin}_{f(X)\geq\tau}|X|.$
\end{problem}

\subsubsection{Analysis of \ea for SC}
\label{section:eascanalysis}
The approximation result on the algorithm \ea for SC is now presented. Notice that
in contrast to the analysis of \ea for SM presented in Theorem \ref{theorem:ea},
it is not the approximation ratio that is in expectation, but instead the feasibility.
The proof and further discussion of Theorem \ref{theorem:easc} can be found in Section
\ref{appendix:cover} of the appendix.
\begin{theorem}
  \label{theorem:easc}
  Suppose we have an instance of SC with optimal solution $A^*$.
  Let $P=n$, $\delta\in(0,1]$,
  and \eascT.
  Then if \ea is run with
  these inputs and $\mathcal{S}$ is its pool at completion,
  $\ex{f(A)} \geq (1-\delta)^2\tau$
  where
  $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq \ln(1/\delta)|A^*|}f(X).$
\end{theorem}

\subsubsection{\beascl (\beasc)}
The approximation result on \beascl (\beasc), an alternative version of \bea for SC,
is presented in this section.
Recall that in \bea in Section \ref{section:bea} that $\beta$ is advanced if $\ell$ has been
incremented $n/\kappa\ln(1/\epsilon)$ many times.
A difficulty with applying \bea to SC is that the cardinality of the optimal solution
(\budget in SM) is unknown.
\beasc is like \bea, but \beasc makes \maxpointersimple guesses for $|A^*|$,
each with a corresponding $\beta_i$, thus is biased towards \maxpointersimple many solutions in
its pool instead of just one as in \bea.
A description of \beasc can be found in Section \ref{appendix:cover} in the appendix.
%The $\beta_i$ corresponding to the closest
%lower bound of $|A^*|$ is chosen with probability $p/\maxpointer$, resulting in a
%$\maxpointer$ slow down compared to \bea.
\begin{theorem}
  \label{theorem:beasc}
  Suppose we have an instance of SC with optimal solution $A^*$ such that
  $|A^*|\geq 2$.
  Let $P=n$, $\delta\in(0,1]$, \defineepsilon, \definexi, and \beascT
  Then if \beasc is run with
  these inputs and $\mathcal{S}$ is its pool at completion,
  $\ex{f(A)} \geq (1-1/n)(1-\delta)\tau$
  where
  $A=\text{argmax}_{X\in\mathcal{S}, |X|\leq \ln(1/\delta)/(1-\epsilon)|A^*|}f(X).$
\end{theorem}

%\beasc is a version of \bea for SC that does not require knowledge of $|A^*|$.
%It is proven in Section \ref{section:beascanalysis} that \beasc finds approximate solutions that are
%near feasible in expectation for SC in \beasctime time.
%To the best of our knowledge, there does not yet exist an \sg analogue proposed for
%SC, and thus \beasc is the first \beasctime time algorithm analyzed for SC.
%\beasc is like \bea, but is biased towards \maxpointersimple many solutions in
%its pool, each corresponding to an estimate of $|A^*|$.
%The algorithm \beasc is described in Section \ref{section:beascoverview} and pseudocode
%for \beasc is provided in Section \ref{appendix:beasc} in the appendix.

%\subsubsection{Overview of \beasc}
%\label{section:beascoverview}
%\beasc (Algorithm \ref{algorithm:beasc} in Section \ref{appendix:beasc} in the appendix)
%is similar to \bea, and therefore only the differences between \beasc and \bea
%are described here.
%In addition to the parameters of \bea, \beasc requires the parameter \definexi.
%\beasc keeps track of variables $\beta^i$ \alli.
%\selectbeasc returns an element of $\pool$ of cardinality $\beta^i$, where $i$ is chosen
%uniformly randomly (there always exists one), with probability $p$,
%and otherwise chooses uniformly randomly from $\pool$.
%Initially, $\beta^i=0$ \alli.
%$\beta^i$ is incremented when the following conditions have been met on \Hi many times:
%\selectbeasc results in the selection of the element in $\pool$ is cardinality
%$\beta^i$, and \mutate resulted in the flipped membership of a
%single element.
%The details of \beasc, as well as the subroutine \selectbeasc
%can be found in Algorithm \ref{algorithm:beasc} of Section \ref{appendix:beasc} in the appendix.
%It should be noted that \beasc is not equivalent to running a separate \bea with $\beta=\beta^i$ for
%each $i$, because there is one pool $\pool$ that is being shared.

%\subsubsection{Analysis of \beasc for SC}
%\label{section:beascanalysis}
%The approximation results of \beasc for SC are now presented.
%In contrast to Theorem \ref{theorem:bea}, it is the feasibility that is in expectation.
%Recall that in \bea in Section \ref{section:bea} that $\beta$ is advanced if $\ell$ has been
%incremented $n/\kappa\ln(1/\epsilon)$ many times.
%A difficulty with applying \bea to SC is that the cardinality of the optimal solution
%(\budget in SM) is unknown.
%This difficulty is ameliorated in \beasc by making $\maxpointer$ guesses for $|A^*|$,
%each with a corresponding $\beta_i$. The $\beta_i$ corresponding to the closest
%lower bound of $|A^*|$ is chosen with probability $p/\maxpointer$, resulting in a
%$\maxpointer$ slow down compared to \bea.

%The proof of Theorem \ref{theorem:easc} uses a related argument to Theorem \ref{theorem:ea}
%where the variables $\omega$ and $\beta$ are tracked (See Section \ref{section:ea} for
%definitions). But instead, the expected time until $\omega$ reaches $\min\{n,\ln(1/\delta)|A^*|\}$
%time is proven to be \easctime. If $\omega \geq \min\{n,\ln(1/\delta)|A^*|\}$,
%then $\ex{f(X)} \geq (1-\delta)\tau$ where $|X|=\beta$. The result then follows from the Chernoff bound.

%\input{Sections/Theoretical/Theorems/easc}

%\input{Sections/Theoretical/beasc}

